Finding Zeros: Greedy Detection of Holes

In this paper, motivated by the setting of white-space detection [1], we present theoretical and empirical results for detection of the zero-support E of x \in Cp (xi = 0 for i \in E) with reduced-dimension linear measurements. We propose two low- complexity algorithms based on one-step thresholding [2] for this purpose. The second algorithm is a variant of the first that further assumes the presence of group-structure in the target signal [3] x. Performance guarantees for both algorithms based on the worst- case and average coherence (group coherence) of the measurement matrix is presented along with the empirical performance of the algorithms.

==> refs.bib.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Andrew Harms at 2013-01-26 13:39:29 -0500 


%% Saved with string encoding Unicode (UTF-8) 



@article{yaoMUDjournal2013,
	Author = {Y. Xie and Y. C. Eldar and A. Goldsmith},
	Date-Added = {2013-01-26 15:59:06 +0000},
	Date-Modified = {2013-01-26 18:39:29 +0000},
	Journal = {{IEEE} Trans. Inf. Theory},
	Title = {Reduced-Dimension Multiuser Detection},
	Year = {in press, 2013}}

@conference{BajwaMixon2013,
	Author = {W. U. Bajwa nd D. G. Mixon},
	Booktitle = {Allerton Conf. Comm., Control, Comp.},
	Date-Added = {2013-01-21 17:15:44 +0000},
	Date-Modified = {2013-01-21 17:17:18 +0000},
	Title = {Group Model Selection Using Marginal Correlations: The good, the bad, and the ugly},
	Year = {2013}}

@article{bigdataScience,
	Author = {R. G. Baraniuk},
	Journal = {Science},
	Number = {6018},
	Pages = {717-719},
	Title = {More Is Less: Signal processing and the data deluge},
	Volume = {331},
	Year = {2011}}

@article{CRT2006,
	Author = {E. J. Cand\`es and J. Romberg and T. Tao},
	Date-Modified = {2013-01-26 18:38:02 +0000},
	Journal = {{IEEE} Trans. Inf. Theory},
	Number = {2},
	Pages = {489-509},
	Title = {Robust Uncertainty Principles: Exact Signal Reconstruction From Highly Incomplete Frequency Information},
	Volume = {52},
	Year = {2006}}

@article{troppComputation,
	Author = {J. A. Tropp and S. J. Wright},
	Journal = {Proc. of the {IEEE}},
	Number = {6},
	Pages = {948-958},
	Title = {Computational Methods for Sparse Solution of Linear Inverse Problems},
	Volume = {98},
	Year = {2010}}

@article{a2iteamnus,
	Author = {M. Wakin and S. Becker and E. Nakamura and M. Grant and E. Sovero and D. Ching and J. Yoo amd J. Romberg and A. Emami-Neyestanak and E. Cand\`es},
	Journal = {J. Emerg. Sel. Topics Circ. Syst.},
	Number = {3},
	Title = {A Non-Uniform Sampler for Wideband Spectrally-Sparse Environments},
	Volume = {2},
	Year = {2012}}

@article{rmpi_inp,
	Author = {J. Yoo and C. Turnes and E. Nakamura and C. Le and S. Becker and E. Sovero and M. Wakin and M. Grant and J. Romberg and A. Emami-Neyestanak and E. Cand\`es},
	Journal = {J. Emerg. Sel. Topics Circ. Syst.},
	Number = {3},
	Title = {A Compressed Sensing Parameter Extraction Platform for Radar Pulse Signal Acquisition},
	Volume = {2},
	Year = {2012}}

@inproceedings{rmpi_icassp,
	Address = {Kyoto, Japan},
	Author = {J. Yoo and S. Becker and M. Loh and M. Monge and E. Cand\`es and A. Emami-Neyestanak},
	Booktitle = {Proc. Int. Conf. Acoust. Speech, Signal Process.},
	Pages = {5325-5328},
	Title = {Design and Implementation of a Fully Integrated Compressed-Sensing Signal Acquisition System},
	Year = {2012}}

@unpublished{rmpi_rfic,
	Author = {J. Yoo and S. Becker and M. Loh and M. Monge and E. Cand\`es and A. Emami-Neyestanak},
	Note = {Proc. IEEE Radio Freq. Integr. Circ. Conf.},
	Pages = {31-34},
	Title = {A 100{MHz}-2{GHz} 12.5x sub-{N}yquist rate receiver in 90nm {CMOS}},
	Year = {2012}}

@unpublished{sirjsp2012,
	Author = {A. Khajehnejad and J. Yoo and A. Emami-Neyestanak and B. Hassibi},
	Note = {to be submitted to the J. of Sig. Proc.},
	Title = {A Practical Sublinear Recovery Algorithm for Compressed Sensing},
	Year = {2012}}

@inproceedings{siricassp2012,
	Address = {Kyoto, Japan},
	Author = {J. Yoo and A. Khajehnejad and B. Hassibi and A. Emami-Neyestanak},
	Booktitle = {Proc. Int. Conf. on Acoustics Speech and Sig. Processing},
	Title = {An Analog Sub-Linear Time Sparse Signal Acquisition Framework Based on Structured Matrices},
	Year = {2012}}

@inproceedings{sirisit2011,
	Author = {A. Khajehnejad and J. Yoo and A. Anandkumar and B. Hassibi},
	Booktitle = {Proc. {IEEE} Int. Symp. on Information Theory},
	Pages = {1427-1431},
	Title = {Summary Based Structures with Improved Sublinear Recovery for Compressed Sensing},
	Year = {2011}}

@article{rauhutSCS,
	Author = {H. Rauhut},
	Journal = {Theoretical Foundations and Numerical Methods for Sparse Recovery},
	Pages = {1-92},
	Title = {Compressive sensing and structured random matrices},
	Volume = {9},
	Year = {2010}}

@unpublished{bajwaGabor2010,
	Author = {W. U. Bajwa and A. R. Calderbank and S. Jafarpour},
	Note = {arXiv:1006.0719},
	Title = {Why Gabor Frames? Two Fundamental Measures of Coherence and Their Role in Model Selection},
	Year = {2010}}

@article{bajwaAvgCoherence,
	Author = {W. U. Bajwa and A. R. Calderbank and D. G. Mixon},
	Journal = {J. Appl. and Comp. Harm. Anal.},
	Number = {1},
	Pages = {58-78},
	Title = {Two Are Better Than One: Fundamental parameters of frame coherence},
	Volume = {33},
	Year = {2012}}

@unpublished{bajwaGroup,
	Author = {W. U. Bajwa and D. Mixon},
	Note = {arXiv:1210.2440},
	Title = {Group Model Selection Using Marginal Correlations: The Good, the Bad and the Ugly},
	Year = {2012}}

@inproceedings{bajwaGroupThresholding,
	Address = {Allerton},
	Author = {W. U. Bajwa and A. R. Calderbank and S. Jafarpour},
	Booktitle = {Proc. Comm. Control and Comp.},
	Title = {Revisiting Model Selection And Recovery of Sparse Signals Using One-Step Thresholding},
	Year = {2010}}

@article{troppOMP,
	Author = {J. A. Tropp and A. C. Gilbert},
	Date-Modified = {2013-01-26 18:39:11 +0000},
	Journal = {{IEEE} Trans. Inf. Theory},
	Number = {12},
	Pages = {4655-4666},
	Title = {Signal Recovery From Random Measurements Via Orthogonal Matching Pursuit},
	Volume = {53},
	Year = {2007}}

@inproceedings{harmsRapid2012,
	Author = {A. Harms and W. U. Bajwa and R. Calderbank},
	Booktitle = {Proc. of Asilomar Conference Signals, Systems, and Computers},
	Date-Modified = {2013-01-26 18:35:34 +0000},
	Title = {Rapid Sensing of Underutilized, Wideband Spectrum Using the Random Demodulator},
	Year = {2012}}

@article{harmsCRD,
	Author = {H. A. Harms and W. U. Bajwa and A. R. Calderbank},
	Journal = {{IEEE} Trans. on Sig. Proc.},
	Number = {99},
	Pages = {1},
	Title = {Beating Nyquist Through Correlations: A constrained random demodulator for sampling of sparse bandlimited signals},
	Volume = {PP},
	Year = {2012}}

@inproceedings{yaoMUD2010,
	Address = {Allerton},
	Author = {Y. Xie and A. Goldsmith and Y. C. Eldar},
	Booktitle = {Proc. of Conference on Comm., Control, and Comp.},
	Title = {Reduced-Dimension Multiuser Detection},
	Year = {2010}
}
@article{kerdockZ4,
author={A. R. Calderbank and P. J. Cameron and W. M. Kantor and J. J. Seidel},
title={{$\Z^4$}-Kerdock Codes, Orthogonal Spreads, and Extremal Euclidean Line-Sets},
journal={Proc. London Math. Soc.},
volume={75},
number={2},
pages={436-480},
year={1997}
} 

@techreport{pcast,
author={P. C. Advisors on Science and Technology},
title={Realizing the Full Potential of Government-Held Spectrum to Spur Economic Growth},
institution={Executive Office of the President},
year={July, 2012}
} 

@online{fccWeb,
author={Federal Communications Commision},
title={White Space},
year={2013},
url={http://www.fcc.gov/topic/white-space}
} 











==> refs_rename2refs.bib.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Andrew Harms at 2013-01-26 13:39:29 -0500 


%% Saved with string encoding Unicode (UTF-8) 



@article{yaoMUDjournal2013,
	Author = {Y. Xie and Y. C. Eldar and A. Goldsmith},
	Date-Added = {2013-01-26 15:59:06 +0000},
	Date-Modified = {2013-01-26 18:39:29 +0000},
	Journal = {{IEEE} Trans. Inf. Theory},
	Title = {Reduced-Dimension Multiuser Detection},
	Year = {in press, 2013}}

@conference{BajwaMixon2013,
	Author = {W. U. Bajwa nd D. G. Mixon},
	Booktitle = {Allerton Conf. Comm., Control, Comp.},
	Date-Added = {2013-01-21 17:15:44 +0000},
	Date-Modified = {2013-01-21 17:17:18 +0000},
	Title = {Group Model Selection Using Marginal Correlations: The good, the bad, and the ugly},
	Year = {2013}}

@article{bigdataScience,
	Author = {R. G. Baraniuk},
	Journal = {Science},
	Number = {6018},
	Pages = {717-719},
	Title = {More Is Less: Signal processing and the data deluge},
	Volume = {331},
	Year = {2011}}

@article{CRT2006,
	Author = {E. J. Cand\`es and J. Romberg and T. Tao},
	Date-Modified = {2013-01-26 18:38:02 +0000},
	Journal = {{IEEE} Trans. Inf. Theory},
	Number = {2},
	Pages = {489-509},
	Title = {Robust Uncertainty Principles: Exact Signal Reconstruction From Highly Incomplete Frequency Information},
	Volume = {52},
	Year = {2006}}

@article{troppComputation,
	Author = {J. A. Tropp and S. J. Wright},
	Journal = {Proc. of the {IEEE}},
	Number = {6},
	Pages = {948-958},
	Title = {Computational Methods for Sparse Solution of Linear Inverse Problems},
	Volume = {98},
	Year = {2010}}

@article{a2iteamnus,
	Author = {M. Wakin and S. Becker and E. Nakamura and M. Grant and E. Sovero and D. Ching and J. Yoo amd J. Romberg and A. Emami-Neyestanak and E. Cand\`es},
	Journal = {J. Emerg. Sel. Topics Circ. Syst.},
	Number = {3},
	Title = {A Non-Uniform Sampler for Wideband Spectrally-Sparse Environments},
	Volume = {2},
	Year = {2012}}

@article{rmpi_inp,
	Author = {J. Yoo and C. Turnes and E. Nakamura and C. Le and S. Becker and E. Sovero and M. Wakin and M. Grant and J. Romberg and A. Emami-Neyestanak and E. Cand\`es},
	Journal = {J. Emerg. Sel. Topics Circ. Syst.},
	Number = {3},
	Title = {A Compressed Sensing Parameter Extraction Platform for Radar Pulse Signal Acquisition},
	Volume = {2},
	Year = {2012}}

@inproceedings{rmpi_icassp,
	Address = {Kyoto, Japan},
	Author = {J. Yoo and S. Becker and M. Loh and M. Monge and E. Cand\`es and A. Emami-Neyestanak},
	Booktitle = {Proc. Int. Conf. Acoust. Speech, Signal Process.},
	Pages = {5325-5328},
	Title = {Design and Implementation of a Fully Integrated Compressed-Sensing Signal Acquisition System},
	Year = {2012}}

@unpublished{rmpi_rfic,
	Author = {J. Yoo and S. Becker and M. Loh and M. Monge and E. Cand\`es and A. Emami-Neyestanak},
	Note = {Proc. IEEE Radio Freq. Integr. Circ. Conf.},
	Pages = {31-34},
	Title = {A 100{MHz}-2{GHz} 12.5x sub-{N}yquist rate receiver in 90nm {CMOS}},
	Year = {2012}}

@unpublished{sirjsp2012,
	Author = {A. Khajehnejad and J. Yoo and A. Emami-Neyestanak and B. Hassibi},
	Note = {to be submitted to the J. of Sig. Proc.},
	Title = {A Practical Sublinear Recovery Algorithm for Compressed Sensing},
	Year = {2012}}

@inproceedings{siricassp2012,
	Address = {Kyoto, Japan},
	Author = {J. Yoo and A. Khajehnejad and B. Hassibi and A. Emami-Neyestanak},
	Booktitle = {Proc. Int. Conf. on Acoustics Speech and Sig. Processing},
	Title = {An Analog Sub-Linear Time Sparse Signal Acquisition Framework Based on Structured Matrices},
	Year = {2012}}

@inproceedings{sirisit2011,
	Author = {A. Khajehnejad and J. Yoo and A. Anandkumar and B. Hassibi},
	Booktitle = {Proc. {IEEE} Int. Symp. on Information Theory},
	Pages = {1427-1431},
	Title = {Summary Based Structures with Improved Sublinear Recovery for Compressed Sensing},
	Year = {2011}}

@article{rauhutSCS,
	Author = {H. Rauhut},
	Journal = {Theoretical Foundations and Numerical Methods for Sparse Recovery},
	Pages = {1-92},
	Title = {Compressive sensing and structured random matrices},
	Volume = {9},
	Year = {2010}}

@unpublished{bajwaGabor2010,
	Author = {W. U. Bajwa and A. R. Calderbank and S. Jafarpour},
	Note = {arXiv:1006.0719},
	Title = {Why Gabor Frames? Two Fundamental Measures of Coherence and Their Role in Model Selection},
	Year = {2010}}

@article{bajwaAvgCoherence,
	Author = {W. U. Bajwa and A. R. Calderbank and D. G. Mixon},
	Journal = {J. Appl. and Comp. Harm. Anal.},
	Number = {1},
	Pages = {58-78},
	Title = {Two Are Better Than One: Fundamental parameters of frame coherence},
	Volume = {33},
	Year = {2012}}

@unpublished{bajwaGroup,
	Author = {W. U. Bajwa and D. Mixon},
	Note = {arXiv:1210.2440},
	Title = {Group Model Selection Using Marginal Correlations: The Good, the Bad and the Ugly},
	Year = {2012}}

@inproceedings{bajwaGroupThresholding,
	Address = {Allerton},
	Author = {W. U. Bajwa and A. R. Calderbank and S. Jafarpour},
	Booktitle = {Proc. Comm. Control and Comp.},
	Title = {Revisiting Model Selection And Recovery of Sparse Signals Using One-Step Thresholding},
	Year = {2010}}

@article{troppOMP,
	Author = {J. A. Tropp and A. C. Gilbert},
	Date-Modified = {2013-01-26 18:39:11 +0000},
	Journal = {{IEEE} Trans. Inf. Theory},
	Number = {12},
	Pages = {4655-4666},
	Title = {Signal Recovery From Random Measurements Via Orthogonal Matching Pursuit},
	Volume = {53},
	Year = {2007}}

@inproceedings{harmsRapid2012,
	Author = {A. Harms and W. U. Bajwa and R. Calderbank},
	Booktitle = {Proc. of Asilomar Conference Signals, Systems, and Computers},
	Date-Modified = {2013-01-26 18:35:34 +0000},
	Title = {Rapid Sensing of Underutilized, Wideband Spectrum Using the Random Demodulator},
	Year = {2012}}

@article{harmsCRD,
	Author = {H. A. Harms and W. U. Bajwa and A. R. Calderbank},
	Journal = {{IEEE} Trans. on Sig. Proc.},
	Number = {99},
	Pages = {1},
	Title = {Beating Nyquist Through Correlations: A constrained random demodulator for sampling of sparse bandlimited signals},
	Volume = {PP},
	Year = {2012}}

@inproceedings{yaoMUD2010,
	Address = {Allerton},
	Author = {Y. Xie and A. Goldsmith and Y. C. Eldar},
	Booktitle = {Proc. of Conference on Comm., Control, and Comp.},
	Title = {Reduced-Dimension Multiuser Detection},
	Year = {2010}
}
@article{kerdockZ4,
author={A. R. Calderbank and P. J. Cameron and W. M. Kantor and J. J. Seidel},
title={{$\Z^4$}-Kerdock Codes, Orthogonal Spreads, and Extremal Euclidean Line-Sets},
journal={Proc. London Math. Soc.},
volume={75},
number={2},
pages={436-480},
year={1997}
} 

@techreport{pcast,
author={P. C. Advisors on Science and Technology},
title={Realizing the Full Potential of Government-Held Spectrum to Spur Economic Growth},
institution={Executive Office of the President},
year={July, 2012}
} 

@online{fccWeb,
author={Federal Communications Commision},
title={White Space},
year={2013},
url={http://www.fcc.gov/topic/white-space}
} 










